Forget-Me-Not: Learning to Forget in Text-to-Image Diffusion Models

The unlearning problem of deep learning models, once primarily an academic concern, has become a prevalent issue in the industry. The significant advances in text-to-image generation techniques have prompted global discussions on privacy, copyright, and safety, as numerous unauthorized personal IDs, content, artistic creations, and potentially harmful materials have been learned by these models and later utilized to generate and distribute uncontrolled content. To address this challenge, we propose \textbf{Forget-Me-Not}, an efficient and low-cost solution designed to safely remove specified IDs, objects, or styles from a well-configured text-to-image model in as little as 30 seconds, without impairing its ability to generate other content. Alongside our method, we introduce the \textbf{Memorization Score (M-Score)} and \textbf{ConceptBench} to measure the models' capacity to generate general concepts, grouped into three primary categories: ID, object, and style. Using M-Score and ConceptBench, we demonstrate that Forget-Me-Not can effectively eliminate targeted concepts while maintaining the model's performance on other concepts. Furthermore, Forget-Me-Not offers two practical extensions: a) removal of potentially harmful or NSFW content, and b) enhancement of model accuracy, inclusion and diversity through \textbf{concept correction and disentanglement}. It can also be adapted as a lightweight model patch for Stable Diffusion, allowing for concept manipulation and convenient distribution. To encourage future research in this critical area and promote the development of safe and inclusive generative models, we will open-source our code and ConceptBench at \href{https://github.com/SHI-Labs/Forget-Me-Not}{https://github.com/SHI-Labs/Forget-Me-Not}.

==> figures/figure_attention_mp.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{assets/attn-map.pdf}
    \caption{An illustration of attention score matrix obtained from cross attention. Scores enclosed in red rectangle indicates the attention paid by pixels to inverted concept, which our method minimizes.}
    \vspace{-0.5cm}
    \label{fig:attention-mp}
\end{figure}

==> figures/figure_baseline.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{assets/baseline.pdf}
    \caption{Finetuning to forget concept "Johnny Depp" with unrelated images of "a photo of man". This method distorts other concepts with visual details of selected unrelated images.}
    \vspace{-0.3cm}
    \label{fig:baseline}
\end{figure}


==> tex/4_conceptbench_deprecated.tex <==
Though there are many benchmarks~\cite{lin2014microsoft, saharia2022photorealistic} to evaluate the generation ability of text-to-image models, none of them measures the memorization of a certain concept. To evaluate the level of memorization and the influence to other concepts, we propose a new benchmark, \textbf{ForgetBench}. ForgetBench consists of eight most representative categories in LAION~\cite{schuhmann2022laion} dataset. For each category, we select six representative instances which can be generated with high fidelity in Stable Diffusion v2-1~\cite{Rombach_2022_CVPR}, shown in Figure~\ref{fig:forgetbench}. Since we aim to evaluation the connection between a concept prompt and generated images, it's nature to select concepts that can be generated in the original model with high fidelity. 

We choose person and animation categories because they are two of the most common cases that may cause privacy or copyright dispute. In person category, we select instances considering the diversity and frequency in LAION dataset. While in animation category, we select famous instances of different styles. Some characters such as iron man or superman even have realistic figures, which makes it interesting to explore the relationship between the textual concept and the visual representation. Furthermore, we select hierarchical instances in animal and plant categories. Specifically, the animal category includes both coarse instance of dog and fine instance of husky. 

Concepts are not limited to concrete objects but also abstract styles or relations. To evaluate these abstract concepts, ForgetBench also includes style category and relation category. 


\begin{figure*}
    \centering
    \setlength{\tabcolsep}{0.5pt}
    \renewcommand{\arraystretch}{0.3}
    {\small
    \begin{tabular}{c@{\hspace{0.1cm}} c c c c c c}

        & Elon Musk & Taylor Swift & Barack Obama & Bill Gates & Johnny Depp & Donald Trump \\
        {\raisebox{0.35in}{
        \rotatebox{90}{\begin{tabular}{c} Person \end{tabular}}}} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/Elon_Musk.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/taylor_swift.JPEG} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/barack_obama.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/bill_gates2.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/johnny_depp.JPEG} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/donald_trump.JPEG} \\ \\ \\
        & Mickey Mouse & Superman & Iron Man & Spider Man & Bat Man & Mulan\\
        {\raisebox{0.27in}{
        \rotatebox{90}{\begin{tabular}{c} Animation \end{tabular}}}} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/mickey.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/superman.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/iron_man.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/spider_man.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/bat_man.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/mulan.jpg} \\ \\ \\
        & Corgi & Husky & British Shorthair & Ragdoll & Bird & Dog \\
        {\raisebox{0.35in}{
        \rotatebox{90}{\begin{tabular}{c} Animal \end{tabular}}}} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/corgi.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/husky.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/british_shorthair.JPEG} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/ragdoll.jpg} &
        \includegraphics[width=0.16\textwidth]{example-image-duck} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/dog.jpg} \\ \\ \\
        & Tree & Flower & Apple & Banana & Mango & Orange \\
        {\raisebox{0.42in}{
        \rotatebox{90}{\begin{tabular}{c} Plant \end{tabular}}}} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/tree.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/flower.JPEG} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/apple.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/banana.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/mango.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/orange.jpg} \\ \\ \\
        & van Gogh & Claude Monet & Cyber Punk & Pixel Art & Picasso & Fantasy \\
        {\raisebox{0.4in}{
        \rotatebox{90}{\begin{tabular}{c} Style \end{tabular}}}} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/van_gogh.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/monet.JPG} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/cyber_punk.jpg} &
        \includegraphics[width=0.16\textwidth]{example-image-duck} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/picasso.JPEG} &
        \includegraphics[width=0.16\textwidth]{example-image-duck} \\ \\ \\
        & Ride & In & In front of & On & Beneath & Hold \\
        {\raisebox{0.31in}{
        \rotatebox{90}{\begin{tabular}{c} Relation \end{tabular}}}} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/ride.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/in.jpg} &
        \includegraphics[width=0.16\textwidth]{example-image-duck} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/on2.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/beneath.jpg} &
        \includegraphics[width=0.16\textwidth]{iccv2023AuthorKit/assets/forgetbench/hold.jpg} \\ \\ \\


    \end{tabular}
    
    }
    \vspace{-0.15cm}
    \caption{Qualitative comparison to Composable Diffusion. Composable Diffusion often results in ``hybrid'' objects which mix the subjects in the input prompt. 
    }
    \label{fig:forgetbench}
\end{figure*}
  
% \subsection{Memorization Score}
% To measure the entanglement between the concept prompt and the visual content quantitatively, we propose \textit{memorization score}. The objective of concept forgetting is to decrease the entanglement between the concept prompt and the visual content. Therefore, the similarity between the representation of a concept prompt and the representation of an image can serve as a measure. However, 
% Given a series of concept images, the textual inversion of these images infuses the representation of the visual content. Therefore, the distance between the 
